VoCopilot: Voice-Activated Tracking of Everyday Interactions

Voice plays an important role in our lives by facilitating communication, conveying emotions, and indicating health. Therefore, tracking vocal interactions can provide valuable insight into many aspects of our lives. This paper presents our ongoing efforts to design a new vocal tracking system we call VoCopilot. VoCopilot is an end-to-end system centered around an energy-efficient acoustic hardware and firmware combined with advanced machine learning models. As a result, VoCopilot is able to continuously track conversations, record them, transcribe them, and then extract useful insights from them. By utilizing large language models, VoCopilot ensures the user can extract useful insights from recorded interactions without having to learn complex machine learning techniques. In order to protect the privacy of end users, VoCopilot uses a novel wake-up mechanism that only records conversations of end users. Additionally, all the rest of pipeline can be run on a commodity computer (Mac Mini M2). In this work, we show the effectiveness of VoCopilot in real-world environment for two use cases.

==> Sections/discussion.tex <==
% Our research on VoCopilot has demonstrated promising results in terms of storage efficiency, privacy preservation, transcript accuracy and LLM insights performance. However, there is always room for further enhancement and exploration.

\fakepar{Tracker} In this early work, we have presented the 


Looking ahead, one potential direction could be to investigate the energy consumption of VoCopilot. While VoCopilot can perform KWS accurately, we could optimise the energy and power required by VoCopilot. This could possibly allow for VoCopilot to be continuously powered for days or weeks without being charged, making it more apt for tracking daily vocal interactions. Another potential direction would be to compress the end-to-end system into VoCopilot through leveraging of tinyML. This would enable both the ASR and Local LLM to be deployed into the VoCopilot chip, reducing latency and dependencies on edge devices. Ultimately, our goal is to continue improving VoCopilot, making it an even more effective and reliable tool for users.

